IQA-Adapter: Exploring Knowledge Transfer from Image Quality Assessment to Diffusion-based Generative Models

Diffusion-based models have recently revolutionized image generation, achieving unprecedented levels of fidelity. However, consistent generation of high-quality images remains challenging partly due to the lack of conditioning mechanisms for perceptual quality. In this work, we propose methods to integrate image quality assessment (IQA) models into diffusion-based generators, enabling quality-aware image generation. We show that diffusion models can learn complex qualitative relationships from both IQA models' outputs and internal activations. First, we experiment with gradient-based guidance to optimize image quality directly and show this method has limited generalizability. To address this, we introduce IQA-Adapter, a novel framework that conditions generation on target quality levels by learning the implicit relationship between images and quality scores. When conditioned on high target quality, IQA-Adapter can shift the distribution of generated images towards a higher-quality subdomain, and, inversely, it can be used as a degradation model, generating progressively more distorted images when provided with a lower-quality signal. Under high-quality condition, IQA-Adapter achieves up to a 10% improvement across multiple objective metrics, as confirmed by a user preference study, while preserving generative diversity and content. Furthermore, we extend IQA-Adapter to a reference-based conditioning scenario, utilizing the rich activation space of IQA models to transfer highly specific, content-agnostic qualitative features between images.

==> sec/into_old_old.tex <==
\section{Introduction}
\label{sec:intro}
\begin{figure*}[ht!]
\centering
%\resizebox{.8\textwidth}{}{%
   \includegraphics[width=.77\textwidth]{imgs/Converted_pdfs/2d_viz_converted.pdf}
  \caption{Quality-aware image generation with \textbf{IQA-Adapter}. All images are generated with the SDXL base model, the same prompt, and the seed. The IQA-Adapter is trained with TOPIQ \cite{topiq} and LAION-Aesthetics \cite{laion_aes} metrics.}
  \label{fig:demo_2d}%
%}
\end{figure*}
Recent advances in diffusion-based image generation have led to a new wave of powerful text-to-image models, capable of producing realistic and highly detailed images from text prompts. Models such as DALL-E 3 \cite{betker2023improving}, FLUX \cite{flux}, and SDXL \cite{podellsdxl} exemplify this success, establishing new standards in visual fidelity and alignment with user intent. Beyond text prompts, recent studies have extended the conditioning flexibility of generative models by incorporating additional guidance sources such as depth \cite{zhang2023adding}, pose \cite{zhang2023adding}, and images \cite{ye2023ip-adapter}, expanding the expressive capacity of these models and enabling greater control over generation outputs. This development has also sparked interest in unified approaches, with recent work like OmniGen \cite{xiao2024omnigen} proposing universal models that integrate diverse conditioning types natively.

Despite these advances, one area that remains largely unexplored in the context of conditional generative modeling is image quality and aesthetics assessment (IQA/IAA). IQA, a specialized field within computer vision, focuses on evaluating image quality in ways that align closely with human perception. While closely related, IAA emphasizes aesthetic attributes that are often dependent on the content of the image. In this work, we aim to bridge the gap between generative modeling and IQA/IAA by incorporating IQA-driven conditioning, enabling improvements in generated image quality while preserving content fidelity.
%IQA is a 
%well-established
%field in computer vision dedicated to evaluating image quality in a way that correlates with human perception. 
%By contrast, 
%The field of IAA, though closely related, is more focused on aesthetic properties that are often content-dependent. 
% While IQA primarily addresses lower-level image attributes such as compression artifacts, blurriness, or exposure, IAA encompasses more subjective aspects, such as composition and color harmony, often specific to an image’s content. 
% Although the boundaries between IQA and IAA are not rigid, and the capabilities of IQA/IAA models can vary depending on training datasets, both areas bring valuable insights into how humans assess image quality. 
% Although the boundaries between IQA and IAA are not rigid, both areas bring valuable insights into how humans assess image quality.
%In this work, we bridge the gap between generative modeling and IQA/IAA, leveraging IQA-informed conditioning to enhance generated image quality without losing content fidelity.
% In this work we primarily leverage IQA models, with some input from IAA, to condition image generation in ways that align with human visual preferences.

Aligning generative models with human preferences in terms of image quality has strong practical motivation. While current evaluations 
%quality assessments 
of generative models primarily focus on image-text alignment or distributional closeness to real data, image quality 
has received relatively little attention.
%"in itself"
%--- distinct from textual alignment --- remains less studied. 
Although some recent approaches \cite{xu2024imagereward, Kirstain2023PickaPicAO, wu2023better} have started to address the alignment of generated content with both textual and aesthetic human preferences, very few attempts, if any, have directly incorporated existing IQA/IAA expertise into generative models. This lack of integration persists despite expanding research \cite{fu2024dp, de2024genziqa, li2024feature, wang2024diffusion} that leverages generative priors from diffusion-based models to advance IQA methods, indicating promising potential for knowledge transfer between the fields.
%Although some approaches \cite{xu2024imagereward, Kirstain2023PickaPicAO, wu2023better} have recently explored the alignment of generated content with both textual and aesthetic human preferences, few, if any, efforts have directly integrated existing IQA/IAA knowledge into generative models. This is despite a growing body of work \cite{fu2024dp, de2024genziqa, li2024feature, wang2024diffusion} that draws from the strengths of generative priors of diffusion-based models in developing and refining IQA methods, suggesting a promising potential for knowledge transfer between the two fields.

 %Our approach to knowledge transfer from IQA to diffusion models consists of two main contributions:

%1. Direct IQA-Guided Generation: Our first approach directly incorporates IQA scores into the generative process, using a guidance technique akin to classifier-based guidance methods. Here, we directly optimize the generative model outputs using IQA gradients, aiming for high-quality outputs that conform to IQA criteria. This method serves as a straightforward baseline for IQA-guided generation and offers insights into how IQA models influence quality-driven generation.

%2. IQA-Adapter Architecture: We introduce a novel IQA-Adapter architecture, building on the IP-Adapter framework, which allows the integration of IQA scores into text-to-image diffusion models without modifying the underlying model weights. By conditioning the model on IQA/IAA scores via additional attention mechanisms, the IQA-Adapter enables quality-aware image generation. that can enhance or even degrade image quality based on specified IQA scores. This architecture not only increases image quality by selectively incorporating fine-grained details but also demonstrates the potential to replicate realistic degradations present in the training set. Although a full exploration of IQA-based degradation generation is beyond the scope of this work, we provide visual examples of this use case.

%Additionally, we examine the potential of IQA-conditioned generation to inform and improve adversarial robustness in IQA models. By leveraging IQA-informed guidance, our methods implicitly identify features that contribute to perceived high quality, offering insights into the limitations and adversarial vulnerabilities of IQA models when faced with generated content. 

%Through these contributions, we present the first systematic attempt to integrate IQA knowledge into generative models, advancing the alignment of image generation quality with human visual preferences and establishing a foundation for future research at the intersection of IQA and image generation.

We summarize our contributions as follows:
% \begin{itemize}
%   \item First systematic attempt to transfer knowledge from IQA domain to diffusion models
%   \item Novel IQA-Adapter architecture, that allows conditioning diffusion-based image generation models on image quality
%   \item Comprehensive analysis of quality transfer methods
%   \item Insights into IQA metrics behavior with generated images
% \end{itemize}
\begin{itemize}
\item \textbf{Qualitative adaptation method.} We introduce IQA-Adapter, a novel conditioning tool for diffusion models that enables quality-aware generation guided by IQA/IAA scores. To our knowledge, this work is the first systematic attempt to directly introduce IQA knowledge in a generative setting via conditioning: we show that diffusion models can implicitly learn complex relationships from both IQA models’ outputs and internal activations. %establishing a foundation for further research at the intersection of IQA and generative modeling.
\item \textbf{Diverse IQA/IAA model integration.} We experiment with a range of IQA and IAA models with diverse architectures and training datasets, demonstrating the adaptability of our approach to different quality and aesthetic metrics and the generalization of quality features learned by IQA-Adapter. Furthermore, we employ a gradient-based quality optimization method to explore adversarial patterns that emerge within images generated with a high IQA-guidance scale. %Our findings also shed light on the interactions between IQA models and generated images, identifying features that enhance perceived quality and uncovering potential biases in IQA models.
\item \textbf{Reference-based conditioning.} We adopt IQA-Adapter for qualitative image-prompting scenario, demonstrating that IQA models can be used to transfer highly specific, content-agnostic qualitative features from the reference to a generated image.
\end{itemize}
% \section{Related Work}
% % ниже кусок текста из описания 2 метода, имхо лучше в related work перенести
% Various techniques have been proposed to condition text-to-image generative models on new information from other domains. Some of the most commonly used methods are ControlNets, LoRAs, and adapters. *Low-Rank Adaptation (LoRA)* achieves conditioning by adding trainable low-rank matrices to the weights of transformer-based models, enabling fine-tuning without modifying the base weights significantly. *ControlNets*, in contrast, introduce auxiliary networks to guide the generation process based on specific structures, such as edge maps or depth, but can add notable computational complexity and are primarily suited for structured conditioning.
%-------------------------------------------------------------------------







==> sec/intro_old.tex <==
\section{Introduction}
\label{sec:intro}
\begin{figure*}[ht!]
\centering
%\resizebox{.8\textwidth}{}{%
   \includegraphics[width=.77\textwidth]{imgs/Converted_pdfs/2d_viz_converted.pdf}
  \caption{Quality-aware image generation with \textbf{IQA-Adapter}. All images are generated with the SDXL base model, the same prompt, and the seed. The IQA-Adapter is trained with TOPIQ \cite{topiq} and LAION-Aesthetics \cite{laion_aes} metrics.}
  \label{fig:demo_2d}%
%}
\end{figure*}
Recent advances in diffusion-based image generation have led to a new wave of powerful text-to-image models, capable of producing realistic and highly detailed images from text prompts. Models such as DALL-E 3 \cite{betker2023improving}, FLUX \cite{flux}, and SDXL \cite{podellsdxl} exemplify this success, establishing new standards in visual fidelity and alignment with user intent. Beyond text prompts, recent studies have extended the conditioning flexibility of generative models by incorporating additional guidance sources such as depth \cite{zhang2023adding}, pose \cite{zhang2023adding}, and images \cite{ye2023ip-adapter}, expanding the expressive capacity of these models and enabling greater control over generation outputs. This development has also sparked interest in unified approaches, with recent work like OmniGen \cite{xiao2024omnigen} proposing universal models that integrate diverse conditioning types natively.

Despite these advances, one area that remains largely unexplored in the context of conditional generative modeling is image quality and aesthetics assessment (IQA/IAA). IQA, a specialized field within computer vision, focuses on evaluating image quality in ways that align closely with human perception. While closely related, IAA emphasizes aesthetic attributes that are often dependent on the content of the image. In this work, we aim to bridge the gap between generative modeling and IQA/IAA by incorporating IQA-driven conditioning, enabling improvements in generated image quality while preserving content fidelity.
%IQA is a 
%well-established
%field in computer vision dedicated to evaluating image quality in a way that correlates with human perception. 
%By contrast, 
%The field of IAA, though closely related, is more focused on aesthetic properties that are often content-dependent. 
% While IQA primarily addresses lower-level image attributes such as compression artifacts, blurriness, or exposure, IAA encompasses more subjective aspects, such as composition and color harmony, often specific to an image’s content. 
% Although the boundaries between IQA and IAA are not rigid, and the capabilities of IQA/IAA models can vary depending on training datasets, both areas bring valuable insights into how humans assess image quality. 
% Although the boundaries between IQA and IAA are not rigid, both areas bring valuable insights into how humans assess image quality.
%In this work, we bridge the gap between generative modeling and IQA/IAA, leveraging IQA-informed conditioning to enhance generated image quality without losing content fidelity.
% In this work we primarily leverage IQA models, with some input from IAA, to condition image generation in ways that align with human visual preferences.

Aligning generative models with human preferences in terms of image quality has strong practical motivation. While current evaluations 
%quality assessments 
of generative models primarily focus on image-text alignment or distributional closeness to real data, image quality 
has received relatively little attention.
%"in itself"
%--- distinct from textual alignment --- remains less studied. 
Although some recent approaches \cite{xu2024imagereward, Kirstain2023PickaPicAO, wu2023better} have started to address the alignment of generated content with both textual and aesthetic human preferences, very few attempts, if any, have directly incorporated existing IQA/IAA expertise into generative models. This lack of integration persists despite expanding research \cite{fu2024dp, de2024genziqa, li2024feature, wang2024diffusion} that leverages generative priors from diffusion-based models to advance IQA methods, indicating promising potential for knowledge transfer between the fields.
%Although some approaches \cite{xu2024imagereward, Kirstain2023PickaPicAO, wu2023better} have recently explored the alignment of generated content with both textual and aesthetic human preferences, few, if any, efforts have directly integrated existing IQA/IAA knowledge into generative models. This is despite a growing body of work \cite{fu2024dp, de2024genziqa, li2024feature, wang2024diffusion} that draws from the strengths of generative priors of diffusion-based models in developing and refining IQA methods, suggesting a promising potential for knowledge transfer between the two fields.

 %Our approach to knowledge transfer from IQA to diffusion models consists of two main contributions:

%1. Direct IQA-Guided Generation: Our first approach directly incorporates IQA scores into the generative process, using a guidance technique akin to classifier-based guidance methods. Here, we directly optimize the generative model outputs using IQA gradients, aiming for high-quality outputs that conform to IQA criteria. This method serves as a straightforward baseline for IQA-guided generation and offers insights into how IQA models influence quality-driven generation.

%2. IQA-Adapter Architecture: We introduce a novel IQA-Adapter architecture, building on the IP-Adapter framework, which allows the integration of IQA scores into text-to-image diffusion models without modifying the underlying model weights. By conditioning the model on IQA/IAA scores via additional attention mechanisms, the IQA-Adapter enables quality-aware image generation. that can enhance or even degrade image quality based on specified IQA scores. This architecture not only increases image quality by selectively incorporating fine-grained details but also demonstrates the potential to replicate realistic degradations present in the training set. Although a full exploration of IQA-based degradation generation is beyond the scope of this work, we provide visual examples of this use case.

%Additionally, we examine the potential of IQA-conditioned generation to inform and improve adversarial robustness in IQA models. By leveraging IQA-informed guidance, our methods implicitly identify features that contribute to perceived high quality, offering insights into the limitations and adversarial vulnerabilities of IQA models when faced with generated content. 

%Through these contributions, we present the first systematic attempt to integrate IQA knowledge into generative models, advancing the alignment of image generation quality with human visual preferences and establishing a foundation for future research at the intersection of IQA and image generation.

We summarize our contributions as follows:
% \begin{itemize}
%   \item First systematic attempt to transfer knowledge from IQA domain to diffusion models
%   \item Novel IQA-Adapter architecture, that allows conditioning diffusion-based image generation models on image quality
%   \item Comprehensive analysis of quality transfer methods
%   \item Insights into IQA metrics behavior with generated images
% \end{itemize}
\begin{itemize}
\item \textbf{Advancement in IQA-driven generation.} To our knowledge, this work is the first systematic attempt to employ IQA knowledge in a diffusion-based generation, establishing a foundation for further research at the intersection of IQA and generative modeling.
\item \textbf{IQA-Adapter architecture.} We introduce IQA-Adapter, a novel adapter-based conditioning architecture for diffusion models that enables quality-aware generation guided by IQA/IAA scores. %IQA-Adapter integrates these scores as additional cross-attention inputs, guiding generation toward specified quality levels without significant modification of image content. When conditioned on high-quality scores, it shifts generation towards higher-quality images. Inversely, with low-quality conditions our method can realistically degrade image quality, replicating distortions present in the training data.
\item \textbf{Diverse IQA/IAA model integration.} We experiment with a range of IQA and IAA models with diverse architectures and training datasets, demonstrating the adaptability of our approach to different quality and aesthetic metrics and the generalization of quality features learned by IQA-Adapter. Furthermore, we employ a gradient-based quality optimization method to explore adversarial patterns that emerge within images generated with a high IQA-guidance scale. Our findings also shed light on the interactions between IQA models and generated images, identifying features that enhance perceived quality and uncovering potential biases in IQA models.
%When applied with high scale and target quality, the proposed IQA-Adapter also provides insights into IQA model behavior when interacting with generated images, identifying features that contribute to perceived high quality and revealing potential biases in IQA models.%\item \textbf{ Exploration of IQA Models’ Robustness and Biases}: 
\end{itemize}
% \section{Related Work}
% % ниже кусок текста из описания 2 метода, имхо лучше в related work перенести
% Various techniques have been proposed to condition text-to-image generative models on new information from other domains. Some of the most commonly used methods are ControlNets, LoRAs, and adapters. *Low-Rank Adaptation (LoRA)* achieves conditioning by adding trainable low-rank matrices to the weights of transformer-based models, enabling fine-tuning without modifying the base weights significantly. *ControlNets*, in contrast, introduce auxiliary networks to guide the generation process based on specific structures, such as edge maps or depth, but can add notable computational complexity and are primarily suited for structured conditioning.
%-------------------------------------------------------------------------







==> sec/method_description_old.tex <==
%\section{Proposed Methods}
\section{Learning the relationship between images and visual quality from IQA models}
\begin{figure*}[ht!]
\centering
%\resizebox{.8\textwidth}{}{%
   \includegraphics[width=.8\textwidth]{imgs/Converted_pdfs/overall_scheme_converted.pdf}
  \caption{Overall architecture of the proposed \textbf{IQA-Adapter}. Yellow arrows demonstrate the flow of knowledge from IQA/IAA models to diffusion-based generator.}
  \label{fig:arch}%
%}
\end{figure*}
\subsection{Baselines}
%\subsection{Gradient-based Guidance}
%TODO: сократить вдвое минимум и перенести в саплементари
To establish a simple baseline for integrating IQA model knowledge into the generation process, we introduce a technique inspired by classifier guidance \cite{classguidance}. In our adaptation, we leverage NR-IQA models rather than a classifier, interpreting IQA scores as soft probabilities that reflect the likelihood of an image achieving high perceptual quality. This approach uses feedback from the IQA model to iteratively optimize image quality during the generation process:
$$
\hat{\epsilon}_\theta (z_{t-1}|c_t,f_{\phi})=\epsilon_{\theta}(z_t|c_t) + \alpha \cdot \omega(t)\nabla_{z_t} \log f_{\phi}(D(z_t)),
$$
where $\epsilon_{\theta}$ is a latent diffusion model, $c_t$ is a textual condition, $f_{\phi}$ is a NR metric, $z_t$ represents the latent image at the $t$-th diffusion step, and $D(\cdot)$ is the VAE’s decoder that maps the latent representation back to image space. The parameter $\alpha$ allows adjustment of the IQA guidance weight, balancing the impact of quality conditioning, while the scaling coefficient $\omega(t)$ modulates the gradient's influence over time, linearly increasing from 0 to 1.

Although this method optimizes the target IQA score, its reliance on gradient-based adjustments introduces the risk of exploiting vulnerabilities within the IQA model. This can result in images that receive high ratings from the IQA model yet exhibit noticeable visual distortions --- a phenomenon similar to adversarial attacks, which we further discuss in Section \ref{sec:disc_adv_patterns}. 

Another naive approach involves fine-tuning the generative model on data of the target quality. This method, however, lacks flexibility for controlling the generative process during inference and can affect the generative capabilities of the original model.

% To establish a simple baseline for integrating IQA model knowledge into the generation process, we introduce a technique inspired by classifier guidance\cite{}. Classifier guidance is a commonly used method for conditioning pretrained unconditional generative models with additional information by utilizing gradients from an auxiliary model. Specifically, classifier guidance traditionally involves adding the gradient of the log-probability of a target class, as predicted by a pretrained image classifier, to the noisy image at each diffusion step.%:  
% % $$
% % \text{Formula}
% % $$
% % where \( f \) denotes the classifier model and \( y \) represents the desired class label.

% In our adaptation, we leverage IQA scores rather than class probabilities. IQA scores, normalized to a 0-1 range using min-max scaling, can be interpreted as a soft probability indicating the likelihood of an image achieving high perceptual quality. Thus, we replace the classifier with an IQA model, guiding the generation process through the IQA model’s gradients to achieve quality-aware outputs. This approach uses the IQA model's feedback to iteratively improve image quality during generation.

% However, as the generated image is only partially formed in the early steps of the diffusion process, IQA outputs are less meaningful at these stages. To address this, we introduce a scaling coefficient \( c(t) \) that modulates the gradient's influence over time, gradually increasing from 0 at the start of generation to 1 near the end. This scaling ensures that IQA-based guidance has a stronger impact as the image becomes more defined. Additionally, because IQA models vary in gradient magnitudes, we normalize the guidance coefficient with the gradient’s $L_2$ norm, ensuring consistent guidance strength across different IQA models. The overall IQA-guided generation process can then be formulated as follows:
% $$
% \hat{\epsilon}(z_{t-1}|c_t,f_{\phi})=\epsilon_{\theta}(x_t|c_t)+\alpha \cdot c(t)\nabla_{z_t} \log f_{\phi}(D(z_t)),
% $$
% where $\epsilon_{\theta}$ is a diffusion model, $c_t$ is a text condition, $f_{\phi}$ is a No-Reference IQA model, $z_t$ represents the latent image at the $t$-th diffusion step, and $D(\cdot)$ is the VAE’s decoder that maps the latent representation to image space. The parameter $\alpha$ allows adjustment of the IQA guidance weight, balancing the impact of quality conditioning, and a scaling coefficient $c(t)$ modulates the gradient's influence over time, gradually increasing from 0 to 1.

% While this method optimizes the target IQA score, we also acknowledge potential risks: directly optimizing an image with a model's gradient can expose the IQA model's vulnerabilities. When guidance strength is high, this method may exploit the IQA model, producing images that are rated highly by the IQA model yet visually distorted—a phenomenon similar to adversarial examples. Thus, this technique can also be viewed as a potential white-box adversarial attack on IQA models, a concept we discuss further in Section \ref{} in the context of adversarial robustness in IQA-guided generation.
\subsection{IQA-Adapter}
% \subsection{IQA-Adapter: Learning the relationship between images and visual quality from IQA models}
To address limitations of inference-time gradient optimization, we propose a method that implicitly learns a relationship between images and their corresponding quality assessments. 
By learning this connection, the generative model can internalize features associated with target-quality images and avoid characteristics linked to opposite quality. For instance, when conditioned on high-quality parameters, the model should generate images with fine-grained details and vibrant colors. Conversely, when conditioned on low quality, it should produce artifacts such as JPEG compression distortions or blurring.
%For instance, it should produce more fine-grained details and vivid colors when conditioned on high quality and, inversely, produce distortions like  JPEG-compression artifacts or blur when conditioned on low quality.
%By learning this connection, model should be able to reproduce image features specific to highly rated images and avoid those of low-quality ones.

\subsubsection{Architecture}
% Across various conditioning techniques, we selected adapter architecture for our purposes, as it maintains a lightweight architecture, does not require changes to the core model weights, and introduces minimal computational overhead during training and inference.

To condition the generative model on image quality, we leverage IP-Adapter \cite{ye2023ip-adapter} technique, which supports image-prompt conditioning in pretrained text-to-image diffusion models. The IP-Adapter operates by projecting the CLIP embedding of an image prompt into additional tokens, which are then integrated into the model via cross-attention mechanisms. This method enables the base model to receive detailed conditioning information from non-textual sources without altering its core weights. We selected this architecture for its lightweight design, ability to preserve core model's weights, and minimal computational overhead during training and inference.
%We selected the adapter architecture for our purposes, as it maintains a lightweight architecture, does not require changes to the core model weights, and introduces minimal computational overhead during training and inference.

As illustrated in Figure \ref{fig:arch}, we repurpose the IP-Adapter framework to pass visual quality scores as conditioning information into the generative model. We refer to this modified approach as \textbf{IQA-Adapter}. In this setup, quality scores are projected into tokens matching the dimensionality of textual tokens through a small projection module, consisting of a linear layer and LayerNorm \cite{ba2016layernormalization}. These tokens then enter the main generative model (U-Net in SDXL \cite{podellsdxl}) via cross-attention layers, allowing the model to adjust image quality based on specified IQA scores.

IQA-Adapter can accept multiple IQA scores as input, allowing for the integration of various IQA/IAA models that capture different aspects of image fidelity, e.g., quality in terms of distortions and overall aesthetics of the image. To ensure consistency, all metric values are standardized to have zero mean and unit variance based on the training dataset.
%All metric values are scaled to zero mean and unit variance based on the training dataset. 
%As the quality metrics form a low-dimensional representation (e.g., in a 2D space for quality-aesthetics), we apply positional encoding to enrich these inputs, drawing on a sinusoidal encoding strategy similar to NeRFs. This optional step enhances the model’s sensitivity to nuanced quality variations without affecting behavior at quality extremes:

% \[
% \text{Positional Encoding: } x_i \rightarrow \left[x_i, \sin(2^k \cdot x_i), \cos(2^k \cdot x_i), \ldots\right] \quad \text{for } k = 1, \ldots, L
% \]

% where \(x_1, \ldots, x_n\) are the input quality scores, and \(L\) is the number of additional trigonometric terms.

A key feature of IQA-Adapter, inherited from the IP-Adapter, is its \textbf{Decoupled Cross-Attention} mechanism, which enables the model to process adapter tokens separately from textual prompt tokens. Specifically, the adapter adds an additional cross-attention layer for each existing cross-attention operation in the base model. Without an adapter, the base model processes the textual conditioning \(c_t\) as follows:
$$\operatorname{Attention}(Z, c_t) = \operatorname{Softmax}\left(\frac{Q K^T}{\sqrt{d}}\right) V$$

\noindent where $Q = Z W_q$, $K = c_t W_k$, $V = c_t W_v$, $Z$ are image features and $d$ is the projection space dimension. When the adapter is added, the attention mechanism is modified as follows:
%With the adapter in place, this becomes:
$$\operatorname{DecAttention}(Z, c_t, c_q) = $$
$$\operatorname{Softmax}\left(\frac{Q K^T}{\sqrt{d}}\right) V + \lambda\times\operatorname{Softmax}\left(\frac{Q K'^T}{\sqrt{d}}\right) V' $$

\noindent where $K' = c_q W'_k$, $V' = c_q W'_v$, and $c_q$ are the quality conditioning features. Notably, the query matrix $W_q$ that processes the generated image features $Z$ is shared across both attention operations. This setup allows the IQA-Adapter to learn and apply quality-specific attributes independently from the text-based conditioning and generalize them across various textual contexts. To control the strength of the IQA-Adapter during inference, we introduce a scaling parameter $\lambda$, which adjusts the impact of quality conditioning by modifying the cross-attention term for quality features.

% $$\operatorname{DecAttn}(Z, c_t, c_q) = \operatorname{Attn}(Z, c_t) + \lambda \cdot \operatorname{Attn}(Z, c_q).$$
% As illustrated in Figure \ref{fig:demo_2d} and discussed in Section \ref{sec:}, IQA-Adapter learns quality-related features, producing higher-quality images with characteristics such as increased brightness, contrast, and sharpness when conditioned on high scores. This quality-conditioning capability, combined with the decoupled cross-attention structure, allows the model to generalize quality-specific features across various textual contexts.
% \begin{figure*}[ht!]
% \centering
% %\resizebox{.8\textwidth}{}{%
%    \includegraphics[width=.8\textwidth]{imgs/pdfs/heatmap_new.pdf}
%   \caption{Quality improvement relative to generation without the adapter (in \%) for IQA-Adapters trained on different IQA/IAA models. All IQA-Adapters are conditioned with high target quality (99th percentile of the training dataset) and use the same prompts and seeds. Prompts are taken from Lexica.art user-generated prompts dataset.}
%   \label{fig:heatmap_adapter}%
% %}
% \end{figure*}
\subsubsection{IQA-Adapter Training}
\label{sec:adapter_training}
We train IQA-Adapter on triplets (\text{image}, \text{text}, \text{input quality scores}) where the image-text pairs are drawn from a text-to-image dataset, and the quality scores are estimated by passing each image through a target IQA/IAA model. The training follows the standard denoising diffusion probabilistic model (DDPM) procedure \cite{ho2020denoising}. In this process, a random timestep \(t \sim U[0, 1]\) is sampled, and noise is incrementally applied to the image  $x$ at the corresponding noise scale.
%, where a random timestep \(t \sim U[0, 1]\) is sampled, and the image $x$ is progressively noised at the corresponding noise scale. 
The model then learns to predict the added noise with the following objective:
$$
\mathcal{L} = \mathbb{E}_{x, t, \epsilon} \left[\|\epsilon - \epsilon_\theta(x_t | c_t, c_q)\|^2\right]
$$
where $x_t$ is a noised representation of the input image, \(c_t\) is the textual condition, $c_q$ is the qualitative condition, $\epsilon$ is the added noise, and $\epsilon_\theta(x_t | c_t, c_q)$ is the predicted noise.

During this process, only the adapter weights are adjusted to allow the generative model to incorporate quality score information and steer the output generation accordingly. To maintain flexibility for classifier-free guidance during inference, we randomly drop the textual and quality conditions with a small probability, which encourages the model to generate images unconditionally.

% To train our IQA-Adapter we employ AdamW \cite{loshchilov2019decoupled} optimizer with $\beta_1 = 0.9, \beta_2 =0.999$, and a weight decay of \(1 \times 10^{-2}\). We train IQA-adapter on the CC3M\cite{sharma2018conceptual} dataset ($\sim$3 million images) for 24,000 steps with a learning rate of \(1 \times 10^{-4}\), followed by fine-tuning on the subset of LAION-5B \cite{laion5b} ($\sim$170k images with aesthetics score $>$ 6.5)\cite{} for an additional 3,000 steps with a reduced learning rate of \(1 \times 10^{-5}\). During the primary training phase on CC3M, we use crops of 512$\times$512 resolution and then increase it to 1024$\times$1024 during fine-tuning to match SDXL’s native resolution.

A key advantage of IQA-Adapter is that it does not require backpropagation through the IQA models (as it only uses quality scores of training images), enabling the use of non-differentiable metrics or even ground-truth subjective scores from sufficiently large subjective studies. As demonstrated in Section \ref{sec:hq_cond}, bypassing gradient-based optimization significantly improves the transferability across metrics beyond those used for training, enhancing the generality of the learned quality features across various evaluation models. % This makes IQA-Adapter training a \textit{black-box} approach concerning the target IQA model.

\subsection{Reference-based IQA-Adapter}
In addition to direct conditioning on the target quality level, we also explored the scenario of transferring qualitative information from an existing reference image. For this purpose, we condition a generative model on the activations extracted from the  intermediate layers of an IQA model. More specifically, we apply a pretrained IQA model $f_{\theta}$ to the reference image to extract qualitative embedding $V_{\text{emb}}$, which we then pass through the projection module to obtain qualitative tokens for the subsequent attention operation. We name this variation of the method \textit{Reference-based IQA-Adapter}.

In the conditioning process, we exploit a useful property of activations of some IQA models (especially those from the farthest layers): they contain almost no information about the semantics of the image, but accumulate information necessary for quality assessment (e.g., type and strength of distortions). This allows to extract mostly qualitative, content-agnostic knowledge from the reference image, preventing “leakage” of unwanted information (e.g. objects, faces, colors). In particular, we used the ARNIQA IQA model to obtain qualitative embeddings, whose authors purposefully achieve this property of the activation space using a special training procedure. Our experiments (see Sec. \ref{}) also confirm that it is well-suited for a reference-based scenario.

The training of the reference-based IQA Adapter is similar to the non-reference-based variant: a qualitative embedding is obtained from the image being reconstructed, which is further used as an additional condition for image denoising. In order to expand the coverage of the IQA model’s activation space during adapter training, we also employed an image degradation model introduced in \cite{} as an additional augmentation with a small probability.

\begin{figure*}[ht!]
\centering
%\resizebox{.8\textwidth}{}{%
   \includegraphics[width=.98\textwidth]{imgs/Converted_pdfs/heatmap_with_subj_converted.pdf}
  \caption{(a) Quality improvement relative to generation without the adapter (in \%) for the IQA-Adapters trained on different IQA/IAA models. All IQA-Adapters are conditioned with high target quality (99th percentile of the training dataset) and use the same prompts and seeds. Prompts are taken from Lexica.art user-generated prompts dataset. (b,c) Results of the side-by-side subjective study of the IQA-Adapter conditioned on different quality levels. (b) Overall results of all comparisons. (c) Pair-wise win rates for each quality level. }
  \label{fig:heatmap_adapter}%
%}
\end{figure*}

==> sec/neg_guidance_supp_old.tex <==
\section{Negative Guidance}
\label{sec:neg_guidance}

Since the concept of visual quality has clearly defined notions of "good" and "bad," it becomes feasible to apply \textbf{negative guidance}, akin to its application in text-based generation. Negative guidance for text involves using an additional text prompt that is semantically opposite to the desired outcome. This serves as a conditioning factor in the unconditional part of the generation process:
\begin{equation*}
    \hat{\epsilon}_\theta (z_{t}|c_t, q) 
        = \epsilon_{\theta}(z_t| \varnothing)
        + g \cdot \big(
            \epsilon_{\theta}(z_t| c_t, q)
            - \epsilon_{\theta}(z_t| \varnothing)
        \big)
\end{equation*}
where $\epsilon_{\theta}$ is a latent diffusion model, $g$ is guidance scale, $c_t$ is a textual condition, $q$ is desired quality of image and $\varnothing$ is an empty condition.

This approach pushes the latent representation of the generated image away from producing undesired features described in the negative prompt. 

The standard method for using an IP-Adapter assumes a null-condition in the unconditional part of the noise prediction, as there is no explicit counter-concept for an image prompt. The task of quality conditioning, however, enables defining negative guidance as:
\begin{multline*}
    \hat{\epsilon}_\theta (z_{t}|c_t, q) 
    = \epsilon_{\theta}(z_t| c_t^{\text{neg}}, q^{\text{neg}})
    +  \\
    + g \cdot \big(
        \epsilon_{\theta}(z_t| c_t, q)
        - \epsilon_{\theta}(z_t| c_t^{\text{neg}}, q^{\text{neg}})
    \big)
\end{multline*}
where $q^{\text{neg}}$ specifies a quality level opposite to the desired one and $c_t^{\text{neg}}$ is negative prompt. Since the input scores are normalized with a mean of 0, we can set \(q^{\text{neg}} = -q\). 

Using this approach enhances the adapter's effect, even with moderate adapter strengths. The resulting images become more vivid, sharp, and, in a sense, stylized to align with the ideals of the target metric. Examples of applying negative guidance with various types of negative conditions are presented in Figure~\ref{fig:neg_guidance_good_example}.

Strong negative guidance significantly improves metric scores, with generalization across different metrics. Figure~\ref{fig:neg_guidance_heatmap} shows average improvements increasing from 5-6\% to 8-10\% relative to the base model.
However, strong negative guidance with high adapter scales can result in overly clean, saturated, sharp images, losing fine details (Figure~\ref{fig:neg_guidance_example_supp}). This effect intensifies with higher scales.

These findings emphasize the need for subjective validation, as IQA/IAA models may have biases or vulnerabilities, especially in adversarial scenarios. The generalization of quality improvements suggests shared biases among models, similar to vulnerabilities identified in the VMAF IQA metric~\cite{vmaf, hackvmaf1, Zvezdakova2019HackingVW}. 


\begin{figure*}[ht!]
\centering
%\resizebox{.8\textwidth}{}{%
   \includegraphics[width=.98\textwidth]{imgs/supp_final/pdfs/2d_tiled_viz_neg.pdf}
  \caption{Quality-aware image generation using IQA-Adapter combined with negative guidance. Compared to Figure \ref{fig:demo_2d}, negative guidance exhibits stronger conditioning effect.}
  \label{fig:neg_guidance_good_example}%
%}
\end{figure*}

==> sec/related_work_old.tex <==
\section{Related work}
\label{sec:related_work}

\textbf{Generative Models.} Various approaches have been explored in the field of image generation, including generative adversarial networks (GANs) and variational autoencoders (VAEs), which dominated early progress in the area. Recently, however, diffusion models have emerged as the state-of-the-art approach for image generation. Pioneering works such as \cite{ramesh2021zero, rombach2022high, saharia2022photorealistic} established diffusion models as superior to previous methods,
%demonstrated that diffusion models surpass prior methods,
introducing the first production-grade models capable of generating high-quality images. Following these advancements, further research focused on improving aspects such as image relevance, aesthetic appeal, and overall quality. Studies \cite{liu2024playground, kastryulin2024yaart, dai2023emu, baldridge2024imagen, esser2403scaling, betker2023improving, flux, chen2024pixart} contributed to these improvements through enhancements in data quality, model scaling, architectural refinement, and the exploration of alternative diffusion frameworks.
%Subsequent research \cite{liu2024playground, kastryulin2024yaart, dai2023emu, baldridge2024imagen, esser2403scaling, betker2023improving, flux, chen2024pixart} further improved image generation in terms of relevance, aesthetics, and overall image quality by enhancing data quality, scaling up model sizes, refining architectures and exploring alternative diffusion frameworks.

\textbf{Adapters and customization.} 
Advances in diffusion models have led to the development of new techniques that enhance control over the image generation process. LoRA \cite{hu2022lora} introduced a parameter-efficient fine-tuning method that updates only a low-rank decomposition of model weights, enabling easy model customization and stylization. Methods like Dreambooth \cite{ruiz2023dreambooth} and Textual Inversion \cite{galimage} further enabled personalization by allowing diffusion models to generate outputs tailored to specific user inputs. IP-Adapter \cite{ye2023ip-adapter} extended these works for universal image variation. Additionally, ControlNet \cite{zhang2023adding} and T2IAdapter \cite{mou2024t2i} incorporated spatial conditioning into diffusion models by using supplementary networks to encode specific conditions. Furthermore, ConceptSliders \cite{gandikota2023erasing} introduced an approach for training adapters that can adjust particular attributes within generated images. Most of these techniques, however, focus on conditioning image generation through text, images, or binary masks. In contrast, our work proposes a novel adapter that enables conditioning based on numerical inputs, which represent continuous image attributes such as aesthetics or quality. 
%However, these methods primarily focus on conditioning image generation using text, images, or binary masks. In contrast, we propose a novel adapter capable of conditioning the generation process using numerical inputs that represent continuous image attributes, such as aesthetics or quality.

% Several recent methods explore conditioning on specific technical attributes to guide content generation. For instance, MovieGen \cite{polyak2024movie} conditions video generation on parameters such as camera direction and frame rate, while DIAMOND~\cite{alonso2024diffusion}  encodes keyboard actions to simulate user interactions within a video game. Similarly, SDXL~\cite{podellsdxl} incorporates image size and crop parameters to enhance the pretraining process. However, these methods primarily leverage low-level, technical attributes. In contrast, we propose conditioning on high-level semantic attributes that are automatically extracted from images using pre-trained, task-specific models. 

Several methods explored conditioning on technical attributes to guide content generation, leveraging specific parameters to influence the output \cite{polyak2024movie, alonso2024diffusion, podellsdxl}. For example, SDXL~\cite{podellsdxl} incorporated image size and crop parameters to enhance pretraining. However, these approaches focus primarily on low-level technical attributes. In contrast, our approach introduces conditioning on high-level semantic attributes, which are automatically extracted using pre-trained, task-specific models.

% Several recent methods explore conditioning on specific technical attributes to guide content generation~\cite{polyak2024movie, alonso2024diffusion, podellsdxl}. For example, SDXL~\cite{podellsdxl} incorporates image size and crop parameters to enhance the pretraining process. However, these methods primarily leverage low-level, technical attributes. In contrast, we propose conditioning on high-level semantic attributes that are automatically extracted from images using pre-trained, task-specific models. 

\textbf{IQA and IAA.} Image quality assessment (IQA) focuses on evaluating the technical quality of images by analyzing distortions, artifacts, and other degradations that affect visual perception. IQA methods are typically classified into full-reference (FR) and no-reference (NR) approaches, depending on whether a pristine reference image is available. In contrast, image aesthetics assessment (IAA) deals with subjective judgments about an image's visual appeal, considering factors such as composition, lighting, color harmony, and overall artistic impression. 
% For real-world applications, where such references are rarely present, NR methods are more relevant. Similarly, IAA methods are formulated exclusively in an NR setting.

Early IQA/IAA methods relied on explicitly modeling human perception, scene statistics, or using handcrafted similarity metrics \cite{ssim, ms_ssim, vif, brisque, niqe, diivine, ilniqe}. These approaches were limited by the complexities and incomplete understanding of the human visual system. Modern techniques \cite{hyperiqa, musiq, topiq, dbcnn, arniqa, liqe, tres, yang2022maniqa, cnniqa, clipiqa, nima} have shifted toward machine learning, particularly deep learning models, which are trained on large datasets with human-provided opinion scores \cite{hosu2020koniq, jinjin2020pipal, spaq, clive, flive, ava, kadid, aadb}. Recent advancements also include diffusion-based approaches \cite{fu2024dp, de2024genziqa, li2024feature, wang2024diffusion}, which used generative model priors to enhance the robustness and accuracy of quality assessments. 
Unlike these approaches, which transfer knowledge from generative models to improve IQA, our work reverses this direction by integrating IQA knowledge into diffusion-based generative models, thereby enriching the generative process with quality-focused insights

% Image Quality Assessment aims to measure the technical quality of an image by assessing the extent of image artifacts and distortions. Image Aestetics Assessment (IAA) is a similar task concerned with the subjective perceptions of viewers towards the visual appeal of an image, taking into account aesthetic aspects such as composition, lighting, color harmony, and overall artistic impression.

% According to the requirement for ground-truth reference images, most IQA techniques can be categorized as Full-Reference (FR) or No-Reference (NR). The latter scenario is more relevant for real-world applications. IAA methods exist only in NR formulation.

% Initial assessment methods were based on human perception [], scene statistics [], [], or similarity [] with or without the reference images; however, these methods were limited by our understanding of the human vision system and scene interpretation. Newer approaches [..] relied on training deep learning models on KonIQ \cite{hosu2020koniq}, KADID10k \cite{lin2019kadid}, PIPAL \cite{jinjin2020pipal}, AVA \cite{murray2012ava}, and other IQA or IAA datasets with opinion scores provided by humans. 

% Latest works [...] utilize T2I model’s prior to build stronger and more robust IQA models. GenzIQA train IQA model over cross-attention maps, extracted from finetuned diffusion model. DP-IQA [] utilize pre-trained Stable Diffusion as the backbone, extracting multi-level features from the denoising U-Net guided by prompt embeddings through a tunable text adapter. However, these works consider knowledge transfer from T2I task to IQA task. In contrast, our work considers opposite setting: integration of knowledge from IQA/IAA tasks into T2I generation.
% Some of the latests works on IQA utilize rich generative priors of T2I models to build stronger, more robust and generalizable IQA models.
